A Radio Study of Persistent Radio Sources in Nearby Dwarf Galaxies: Implications for Fast Radio Bursts

We present 1 - 12 GHz Karl G. Jansky Very Large Array observations of 9 off-nuclear persistent radio sources (PRSs) in nearby (z < 0.055) dwarf galaxies, along with high-resolution European very-long baseline interferometry (VLBI) Network (EVN) observations for one of them at 1.7GHz. We explore the plausibility that these PRSs are associated with fast radio burst (FRB) sources by examining their properties, physical sizes, host-normalized offsets, spectral energy distributions (SEDs), radio luminosities, and light curves, and compare them to those of the PRSs associated with FRBs 20121102A and 20190520B, two known active galactic nuclei (AGN), and one likely AGN in our sample with comparable data, as well as other radio transients exhibiting characteristics analogous to FRB-PRSs. We identify a single source in our sample, J1136+2643, as the most promising FRB- PRS, based on its compact physical size and host-normalized offset. We further identify two sources, J0019+1507 and J0909+5955, with physical sizes comparable to FRB-PRSs, but which exhibit large offsets and flat spectral indices potentially indicative of a background AGN origin. We test the viability of neutron star wind nebulae and hypernebulae models for J1136+2643, and find that the physical size, luminosity, and SED of J1136+2643 are broadly consistent with these models. Finally, we discuss the alternative interpretation that the radio sources are instead powered by accreting massive black holes and outline future prospects and follow-up observations for differentiating between these scenarios.

==> extras.tex <==
%The synchrotron SEDs probed in the radio arise from a population of relativistic particles gyrating in a magnetic field, typically following a power-law energy distribution N(E) $\propto$ E$^{-p}$. The radio spectra of PRSs\,20121102A and 20190520B are comparably flat up to frequencies of a few GHz \citep{Chatterjee17, Niu22}. At $\sim$9\,GHz, the spectrum of PRS\,20121102A features a clear break and steepens from $\sim$$\nu^{-0.1}$ to $\sim$$\nu^{-1.3}$ \citep{Chatterjee17,Resmi21}. While the origin of the turnover remains unclear, a plausible explanation is due to synchrotron cooling in which high-energy electrons are depleted at higher frequencies where cooling is efficient, resulting in an accumulation of lower energy electrons that correspond to a spectral break at the cooling frequency $\nu_c$. 

%The flat spectral indices are quite unique among known radio transients. Particles typically gain energy through repeated shock crossings via diffusive shock interactions (DSA; \citealt{Bell78,Blandford87}) which imply an energy index greater than two and a corresponding spectral index steeper than $-$0.5. This is in line with most synchrotron transients including $\gamma$-ray bursts, supernovae, tidal disruption events, and fast blue optical transients \textcolor{red}{CITE}. However, under standard conditions, DSA is unable to explain the flatness in the PRS spectra. 


%%%%%%%%%%%%%SED%%%%%%%%%%%%%%%%%%
%While the study of spectral evolution usually requires contemporaneous observations as fluxes may vary over time, previous studies have found negligible time variability in the light curves of radio transient sources over $\sim$ year timescale at frequencies $<1$\,GHz \citep{Bell14, Rowlinson16}. Thus, for these three sources, we assume that the combination of LoTSS and VLA data represents an SED with data taken on contemporaneous timescales. 
%In Figure \ref{fig:SED}, we highlight the four sources confirmed as compact in grey, and the optically-confirmed AGN sources J1136$+$1252 and J1220$+$3020 in yellow. 

%The emission probed in the radio band is powered by nonthermal, synchrotron radiation \citep{JJCondon92} characterized by a power law (F$_\nu \propto \nu^{\alpha}$) where $\alpha$ is the spectral index with an energy distribution $N(E)\propto E^{-p}$. The expected shape of the SED arises from a population of relativistic particles gyrating in a magnetic field. 


%Usually, steep spectral indices ($\alpha \lesssim -$0.5) in synchrotron SEDs can be explained via diffusive shock interactions (DSA; \citealt{Bell78,Blandford87}) in which particles gain energy through repeated shock crossings. This is in line with most synchrotron transients including supernovae (SNe), tidal disruption events, and fast blue optical transients \citep{Malkov01, Chevalier11, Jiang16, Margutti19, Fang20}. 
%and cannot be explained by diffusive shock interactions (DSA; \citealt{Bell78,Blandford87}) which typically exhibit steep spectral indices with $\alpha \lesssim -$0.5. On the other hand, the flat SEDs are consistent with those of PWNe, with spectral indices generally flatter than $-$0.5 \citep{Gaensler06}. Indeed, such a model has been proposed for PRS\,20121102A \citep{Dai2017, Yang19}. 


%One plausible explanation for the origin of the spectral break is synchrotron cooling in which high-energy electrons are depleted at higher frequencies where cooling is efficient, resulting in an accumulation of lower energy electrons that correspond to a spectral break at the cooling frequency $\nu_c$. 
%On the other hand, the break in the SED of J1136$+$2643 is characterized by a turnover. 

%the synchrotron SEDs probed in the radio band are characterized by a power law with an energy distribution $N(E)\propto E^{-p}$. The shape of the spectrum arises from a population of relativistic particles gyrating in a magnetic field. The particles typically gain energy through repeated shock crossings via diffusive shock interactions (DSA; \citealt{Bell78,Blandford87}) which imply a p $>$ 2 and a corresponding spectral index steeper than $-$0.5. This is in line with most synchrotron transients including $\gamma$-ray bursts (GRBs), supernovae (SNe), tidal disruption events, and fast blue optical transients \citep{Vietri95, Malkov01, Chevalier11, Jiang16, Margutti19, Fang20}.

%For context, the radio SEDs of PRSs\,20121102A and 20190520B are comparably flat up to frequencies of a few GHz \citep{Chatterjee17, Niu22}. At $\sim$9\,GHz, the spectrum of PRS\,20121102A features a clear break and steepens from $\sim$$\nu^{-0.1}$ to $\sim$$\nu^{-1.3}$ \citep{Chatterjee17,Resmi21}. While the origin of the turnover remains unclear, a plausible explanation is due to synchrotron cooling in which high-energy electrons are depleted at higher frequencies where cooling is efficient, resulting in an accumulation of lower energy electrons that correspond to a spectral break at the cooling frequency $\nu_c$. Moreover, the flat spectral indices are quite unique among known radio transients as the energy distribution of the shock-accelerated particles is too hard to by explained by DSA \citep{Blandford87}.


%As demonstrated in Figure \ref{fig:SED}, we find that two-thirds of the radio sources are best characterized by a single power law with spectral indices ranging from $\alpha$ = $-$0.03 to $-$0.92. In particular, J0019$+$1507 exhibits an almost completely flat spectrum, while the spectra of J0106$+$0046 and J0903$+$4824 have steep $\alpha \approx$ $-$1, demonstrating diversity. It is worth noting that J0903$+$4824 is resolved in our VLA observations at low frequencies which was not previously observed in the high-resolution X-band data \citep{Reines20}. Therefore, the shape of the SED is likely a result of two distinct components, unlike the other sources. The flat spectra as observed in Tier B sources (J0019+1507 and J1027+0112) are similar to that of the PRSs. Several theoretical mechanisms can account for the observed flat spectrum. For instance, PWNe are characterized by a spectral index $\alpha$ $<$ $-$0.5 \citep{Gaensler06}, and they have been proposed as a potential explanation for PRS\,20121102A \citep{Dai2017}. However, if we consider the possibility of an off-nuclear BH instead, a flat spectrum may arise from the core when observing an AGN along the jet-axis in which the spectrum is dominated by BH accretion disk nucleus \citep{DeZotti2010}.  Indeed, the presence of a flat spectral shape is apparent in the background AGN, J1136$+$1252.


%Moreover, while none of the sources display an inverted spectral slope, as observed in J1136$+$1252, those in Tiers B and C, characterized by a simple power law, do exhibit a similar shape to the AGN source J1220$+$3020, with comparable spectral indices. Interestingly, J1136$+$1252 is detected with EVN at 1.7\,GHz but not with VLBA at 9\,GHz. A potential explanation is refractive scintillation of the compact core of the background AGN due to small-scale irregularities in the interstellar medium. Indeed, at the galactic latitude of the source, the flux can fluctuate up to 60$\%$ at higher frequencies \citep{Walker98}. We therefore attribute the VLBA non-detection to scintillation-induced variability.


%Next, we examine the four sources exhibiting a broken power law. Among them, half are compact on mas scales, i.e., in Tier A or B. Sources J0909$+$5655 and J1253$-$0312 display two negative spectral indices, indicating a steepening in the spectra after the break frequency. Conversely, J0931$+$5633 in Tier C shows a flat spectral slope followed by a sharp decline above 1\,GHz. We note that it is likely the turnover lies at a lower frequency between 144\,MHz and 1\,GHz. However, the sparse data coverage in this frequency range precludes a more accurate determination of the spectral break. 


% Compare to PRS SEDs
%We now compare the shape of our SEDs to those of PRSs\,20121102A and 20190520B (shown in grey). We construct the SED of PRS\,20121102A with data from the Giant Metre-wave Radio Telescope (GMRT) between 400\,MHz and 1.4\,GHz \citep{Resmi21} and VLA between 1.6 and 22\,GHz \citep{Chatterjee17}. The observations are taken with a temporal separation of up to $\sim$ 1 year at low frequencies. Similarly, we plot the radio spectrum of PRS\,20190520B with VLA data between 1.3 and 6\,GHz \citep{Niu22}. Our frequency coverage limits a direct comparison to both PRSs (Figure \ref{fig:SED}). However, we find that a majority of our sources share a negative spectral slope with both PRSs across the common frequencies between $\sim$ 1 and 6\,GHz. Specifically, the SEDs of Tier B and C sources J1200$-$0341, J1226$+$0815, J1253$-$0312, and J1027$+$0122 are the most consistent with that of PRS\,20190520B while source J0909$+$5655 in Tier B is more closely aligned with PRS\,20121102A


%%%%%%%%%%%%Light Curves%%%%%%%%%%%%%%%%%%%%

%We compile the light curves for the 10 PRS candidates in our sample at 1.4, 3, and 9\,GHz using the radio observations presented in Sections \ref{sec:VLA_obs} and \ref{archival_data}. Additionally, we also include upper limits and detections from archival VLA data for sources J0106$+$0046, J1136$+$2643, and J1200$-$0341 at 1.4 and 9\,GHz as in  \citet{Eftekhari20, Reines20}. The light curves for all 10 PRS candidates are shown in blue (1.4\,GHz), purple (3\,GHz), and orange (9\,GHz) in Figure \ref{fig:LCs}.


% comparison to PRS LCs
% Scintillation stuff
%Based on prevailing progenitor models for FRBs (see Section \ref{sec:models}), PRSs are expected to evolve on timescales of $\sim$ decades to centuries following the supernova explosion that gives rise to a compact central engine. Thus motivated, we examine the light curves at 1.4\,GHz which span the longest temporal baseline ($\sim$ 3 decades). We find that sources J0019$+$1507, J0909$+$4824, J0906$+$5655, and J1253$-$0312 in Tiers B and C are characterized by a monotonic decline. This is contrasted by J0106$+$0046, J1027$+$0112, J1136$+$2643, J1200$-$0341, and J1226$+$0815 which display both a rise and decline in the light curves. Notably, source J1226$+$0815 exhibits the most drastic decrease in flux by a factor of $\sim$ 75$\%$ over a $\sim 20$ year timescale. Among the sources that are compact on mas scales, Tier B sources J0019$+$1507 and J0906$+$5655 show a moderate flux reduction of $\approx$ 40 and 20$\%$ spanning roughly 2 decades, respectively, although the upper limit in the light curve of J0906$+$5655 does not preclude a rise at early times. For compact sources J1027$+$0112 and J1136$+$2643, the fluctuations observed in their light curves are negligible, aligning more closely with a stable, flat temporal evolution. 


%Compared to the decades-long radio transient, J1419$+$3940, the PRS candidates are less luminous than J1419$+$3940 by a factor of 10 at early times. However, our sample sources are fading more gradually than J1419$+$3940 which has a half-peaked decay time of 3 years over 21.5 years \citep{Law18}, As the light curves of J1419$+$3940 is most consistent with an off-axis long GRB, the difference in the decay rate indicates that the sources are powered by a slower-fading emission mechanism such as shock interactions between expanding SN ejecta and the surrounding gas \citep{Metzger15}. We stress that such comparisons cannot be made with the available temporal evolution of the known PRSs as they are discovered too recently to be probed on a decades-long timescale. 


% OLD
%On $\sim$ day timescales, flux density measurements of PRS\,20121102A obtained with the VLA at 3\,GHz \citep{Chatterjee17} show $\sim$ 10$\%$ variability, while observations on a longer $\sim 3$ year baseline at 1.3\,GHz with MeerKAT reveal a 30$\%$ decline in the light curve between 2019 and 2021 \citep{Rhodes23}. The observed short-term temporal variability was attributed to refractive scintillation \citep{Waxman17}, whereas the variability on $\sim$year timescales may be intrinsic to the system (e.g., due to the interaction between a PWN terminal shock and the surrounding supernova ejecta; \citealt{Rhodes23}). Additionally, VLA observations at high frequencies (12 -- 26\,GHz) as observed on a monthly timescale further supported the low level of scintillation variability \citep{Chen23}. For PRS\,20190520B, multi-frequency (1 -- 12\,GHz) monitoring revealed a 20\% decrease in luminosity between 2020 and 2021, alongside marginal variability at 3\,GHz with a 3.2$\sigma$ flux decrease \cite{Zhang23}. 
%Given the recent discovery date of FRB\,20190520B, searches for long-term variability on the same timescale (up to a decade) as observed for PRS\,20121102A are not yet tenable.


%To assess the level of variability for the PRS candidates on shorter $\sim XX$ year timescales, we leverage the light curves at 3 and 9\,GHz. At 3\,GHz, most of the light curves exhibit relatively constant behavior with a moderate variability of $\lesssim$ 20$\%$. An exception is noted in the light curve of J0909$+$5655 (Tier B), which shows a notable rise by a factor of XX over a span of approximately 2 years, followed by a drop in the flux by a factor of XX. Indeed, the light curves of J0106$+$0046 and J1200$-$0341 exhibit a secular decline and are in agreement with that of PRSs. On the other hand, the apparent rise in the light curves of J0909$+$5655 and J0931$+$5633 are inconsistent with what is observed in the PRS light curves and in tension with the model predictions. 

% When compared to the background AGN, the flat spectra Tier B sources mirrors that of J1126$+$1252. If we consider the case of an off-nuclear BH, a flat spectrum may arise from the core when observing an AGN along the jet-axis in which the spectrum is dominated by BH accretion disk nucleus \citep{DeZotti2010}. Indeed, the presence of a flat spectral shape is apparent in the background AGN, J1136$+$1252. 


Navin's model:
%Another paradigm that was proposed to self-consistently explain the properties of the FRB with the PRS involves an accreting stellar-mass compact object that inflates an energetic bubble powered by the outflows (winds and jets) from the super-Eddington accretion disk \citep[`hypernebula';][]{Sridhar+22}. In this picture, the FRB is produced by magnetized shocks or reconnection events at large distances away from the compact object, along the funnel of the jet \citep{Sridhar+21}. Recently, this model has successfully explained the observed properties of FRBs 20210117A \citep{Bhandari+23a}, 20201124A \citep{Dong24}, and 20190520B \citep{Bhandari+23b}; furthermore, the volume-integrated high-energy neutrino emission from hypernebulae could also potentially explain a significant fraction of the observed extragalactic diffuse neutrino flux \citep{Sridhar+24a}. Here, we assess the viability of our Tier A source, J1136$+$2643, being powered by a stellar-mass black hole instead of an intermediate-mass black hole, as inferred by \cite{Reines20}. 

%Let's consider a $30\,M_\star$ star accreting matter onto a black hole of mass $M_\bullet=10\,M_\odot$ at a rate $\dot{M}$. The active lifetime of the system can be approximated as, $t_{\rm active} \approx M_\star/\dot{M}$: this is shown as the golden-brown region in the left panel of Figure~\ref{fig:hypernebulae} for a range of accretion rates normalized to the Eddington accretion rate $\dot{M}_{\rm Edd}\equiv L_{\rm Edd}/(0.1c^2)$, where $L_{\rm Edd}\simeq1.5\times10^{39}\,{\rm erg\,s^{-1}}(M_\bullet/10\,M_\star)$ is the Eddington luminosity. The super-Eddington accretion event is expected to drive large-angled slower winds from the disk with a kinetic luminosity, 

%\begin{equation}
%L_{\rm w}\approx\frac{1}{2}\dot{M}v_{\rm w}^2 \approx 5\times10^{41}\,{\rm erg\,s^{-1}}\left(\frac{\dot{M}}{10^5\,\dot{M}_{\rm Edd}}\right)\left(\frac{M_\bullet}{10\,M_\star}\right)v_{\rm w,9}^2,
%\end{equation}

%where $v_{\rm w,9}=v_{\rm w}/10^9\,{\rm cm\,s^{-1}}$ is the velocity of the wind. %\footnote{Hereafter, we adopt the shorthand notation $Y_{\rm x} \equiv Y/10^{\rm x}$ for quantities given in cgs units.} 
%This wind interacts with the upstream circumstellar medium (with a number density of say, $n_{\rm csm}=10\,{\rm cm^{-3}}$) and accumulates a shell. The time-evolution of the radius of this wind ejecta shell---bridging the free-expansion and decelerating phases---as a function of $\dot{M}$ and $v_{\rm w}$ is given by Equation~10 in \cite{Sridhar+22}. We use the available constraint on the size of J1136$+$2643 being $<1.43$\,pc to rule-out regions of the $\dot{M}$-evolutionary time parameter space (black hatched region in Figure~\ref{fig:hypernebulae}). Assuming that the radio synchrotron emission be produced within this shell, 
%we can rule out the accretion rates and times during the hypernebula's evolution for which the optical depth through the shell to free-free absorption for radio waves at 3\,GHz is $>1$ (blue region in Fig.~\ref{fig:hypernebulae}). These heated electrons efficiently radiate as long as their synchrotron cooling timescale is shorter than their adiabatic cooling timescale, set by the expanding nebula (Eq.~49 of \citealt{Sridhar+22}). The values of $\dot{M}$ and the times that yield an inefficient synchrotron emission is marked by the thistle colored region in Figure~\ref{fig:hypernebulae}: here, we assume the jet magnetization to be $\sigma_{\rm j}=0.1$ (defined as the ratio of the magnetic enthalpy densityto plasma enthalpy density). These constraints are obtained for the fiducial set of parameters (listed in the top right of the figure); this also leaves us with a narrow region in the $\dot{M}$-evolutionary time parameter space (unshaded, white) that we explore further to explain the spectrum of J1136$+$2643.

%The accreting black hole will also drive out much faster winds, with speeds $v_{\rm j}\sim0.4\,c$ along the spin axis (`jet'), with a luminosity $L_{\rm j}\approx\eta L_{\rm w}$, where the jet efficiency is $\eta<1$. The radio synchrotron emission in the hypernebula arises from the collision between the faster jet and the slower disk-wind shell that heats relativistically hot particles behind the shell. The luminosity of the shock-heated electrons is $L_{\rm e}\approx\varepsilon_{\rm e} L_{\rm j}$, where $\varepsilon_{\rm e}\sim0.5$ is the fraction of the heating efficiency of the electrons \citep{Sironi&Spitkovsky_11} in an electron-ion shock with $\sigma_{\rm j}\sim0.1$; the red region in the left panel of Figure~\ref{fig:hypernebulae} rules out the $\dot{M}$ range for the assumed fiducial parameters where $L_{\rm e}\lesssim2\times10^{38}\,{\rm erg\,s^{-1}}$ (which is the observed radio synchrotron luminosity from J1136$+$2643).

%Given these constraints, we construct an `effective multi-zone' model for the observed radio synchrotron spectrum of J1136$+$2643. The right panel of Figure~\ref{fig:hypernebulae} shows the model (dark grey curve) superimposed on the observed spectrum (black dots); also shown for comparison are the spectra of the PRSs associated with FRBs 20121102A and 20190520B (denoted by maroon squares and red diamonds, respectively). The model is constructed taking $\dot{M}/\dot{M}_{\rm Edd}=10^5$ and at 10 years of evolution. This is because, (1) it resembles the parameters derived for explaining the PRSs associated with FRBs 20121102A and 20190520B \citep{Sridhar+22} and (2) the shock is in an efficient synchrotron emission regime. One-zone model radio synchrotron spectra are first produced by varying the following parameters within the ranges: $v_{\rm j}/c\in[0.17,0.3], \eta\in[0.7,1], \varepsilon_{\rm e}\in[0.17,0.5]$ such that $\epsilon_{\rm e}\propto v_{\rm j}$ and $L_{\rm j}\propto \eta v_{\rm j}^2\sim constant$. The final radio spectrum is generated by performing a weighted-sum of the spectral curves from these one-zone models. The specific choice of the weights $w$, is such that $w\propto (\varepsilon_{\rm e}v_{\rm j}^2)^{-2}$, with minor modifications around it to fit the spectra. This approach of a linear weighting of the models is justified by the fact that the shockfront may have different speeds and efficiencies at different regions, and the electrons are injected into the same nebula with different energies (e.g., at different epochs if $v_{\rm j}$ is varying in time, or at different locations if the termination shock properties vary spatially).  The final weighted-spectrum shown in the right panel of Fig.~\ref{fig:hypernebulae} (dark grey curve), reveals a satisfactory (admittedly tuned) proof-of-principle match to the spectrum of J1136$+$2643.

Section 6:
%Furthermore, the flat spectral index ($\alpha \approx -0.03 - -0.20$) observed in the Tier B sources is reminiscent of the flat spectrum radio cores of AGN. The emission from AGN is anisotropic and orientation-dependent due to the discoveries of relativistic jets launched by the central BH \citep{Urry95}. Consequently, when observed close to the jet-axis, the flat SED originates from the compact base of the approaching jet. Similarly, a view down the jet axis offers an unobstructed view of the BH-accretion disk nucleus, also resulting in a flat SED \citep{DeZotti2010}. Indeed, the flat spectra of the Tier B sources mirrors that of the known compact AGN source J1126$+$1252. Thus, the spectral similarities, coupled with the large host-normalized offsets, suggests a potential association between Tier B sources and background AGN. 


Intro (first draft): 
%Fast radio bursts (FRBs) are luminous, short-duration (ms -- s) pulses of coherent radio emission with dispersion measures (DMs) well in excess of the Milky Way contribution, suggesting an extragalactic provenance \citep{Lorimer07, Cordes19, Petroff22, Zhang23Review}. With discoveries growing at a rapid rate and hundreds of events identified thus far \citep{Bannister17, Law18, CHIME_catalog}, FRBs represent a prolific cosmological source population whose origin is still broadly debated. This is primarily due to both the scarcity of well-localized events and the distinction between FRBs which exhibit repeat bursts (``repeaters") \citep{Spitler16} and apparent one-off events (so called ``non-repeaters'', \citealt{Shannon18,CHIME_catalog}). Moreover, the connection of only a handful of FRBs to multi-wavelength counterparts \citep{Scholtz16, Nunez21, Tavani21, Kilpatrick23, Law23} presents further challenge in illuminating the nature of their progenitors.


%At present, the prevalence of PRS emission is uncertain. Moreover, the high volumetric rate of FRBs suggests that PRSs may constitute a new population of extragalactic radio sources \citep{Law22} preferentially located in dwarf host environments and displaced from the galactic nucleus. Indeed, a search for these sources led to the discovery of the decades-long radio transient FIRST J141918.9$+$394036 (hereafter J1419$+$3940) that has been hypothesized as an orphan long $\gamma$-ray burst (LGRB) afterglow \citep{Law18}, the persistent radio emission coincident with the superluminous supernova (SLSN) PTF10hgi \citep{Eftekhari19} nearly a decade after explosion, as well as the pulsar wind nebula (PWN) candidate VLASS transient J113706.19$–$033737.3 (hereafter VT 1137$–$0337; \citealt{DDong23}). The two robust cases of PRS associations underscores their significance for at least some FRBs. Given the diversity of PRS emission, it is therefore imperative to distinguish PRSs particularly associated with FRBs, as they may represent a distinct sub-class in the FRB population and serve as signposts of FRBs.


%The identification of the first repeating FRB\,20121102A pinpointed its location to a low-mass, dwarf host galaxy at $z = 0.1927$ \citep{Chatterjee17, Tendulkar17}. Within the host environment, FRB\,20121102A was found to be co-located with a compact ($\approx 1$~pc) persistent radio source (PRS), and offset from the nucleus of the host galaxy \citep{Marcote17}. To date, several dozen FRBs have been localized to galaxies up to $z\sim1$ \citep{Heintz20,Gordon23, Law23} but only one other definitive FRB-PRS pair, FRB\,20190520B, has been discovered in a dwarf galaxy at $z = 0.241$ \citep{Niu22}, rendering it a close analog to FRB\,20121102A. We note that a third PRS was recently claimed to be associated with the active repeating FRB\,20201124A in a non-dwarf spiral host galaxy \citep{Xu22,Bruni23,Dong24}. However, the apparent offset of the PRS from the FRB location and a lack of definitive evidence as to its compact nature makes this association more tentative.  

 %The presence of PRS emission discovered with FRBs serves as a powerful tool for delineating progenitor formation channels and emission models of FRBs such as neutron star wind nebula \citep{Yang16, Beloborodov17, Margalit18, Li20} and hypernebula \citep{Sridhar+22, Sridhar+24a}. Importantly, their distinctive prevalence in dwarf host environments and displacement from the galactic nucleus may serve as signposts of FRBs. Indeed, similar radio sources have been discovered in nearby dwarf galaxies including the decades-long radio transient FIRST J141918.9$+$394036 (hereafter J1419$+$3940; \citealt{Law18}), the persistent radio emission coincident with the superluminous supernova (SLSN) PTF10hgi \citep{Eftekhari19} nearly a decade after explosion, as well as the pulsar wind nebula (PWN) candidate VLASS transient J113706.19$–$033737.3 (hereafter VT 1137$–$0337; \citealt{DDong23}). Given the diversity of PRS emission, it is therefore imperative to differentiate those associated with FRBs, as they may constitute a unique sub-class in the broader FRB population.

 Draft #2:
 %The recent advancements in radio facilities and observing techniques, exemplified by the VLA has revealed a novel population of extragalactic radio sources associated with explosive phenomena. These radio sources are preferentially located in dwarf host environments and displaced from the galactic nucleus. At present, the prevalence of such persistent radio source (PRS) is uncertain. Moreover, they have also been discovered in a rather heterogeneous way thus far. For example, a targeted search for PRS associated with transients has led to the discoveries of the decades-long radio transient FIRST J141918.9$+$394036 (hereafter J1419$+$3940) that has been hypothesized as an orphan long $\gamma$-ray burst (LGRB) afterglow \citep{Law18} as well as the persistent radio emission coincident with the superluminous supernova (SLSN) PTF10hgi \citep{Eftekhari19} nearly a decade after explosion. Meanwhile, a serendipitous search in the VLA Sky Survey (VLASS; \citealt{VLASS}) has uncovered the pulsar wind nebula (PWN) candidate J113706.19$–$033737.3 (hereafter VT 1137$–$0337; \citealt{DDong23}). 


%Given the diversity in the nature of those PRS emission, it is therefore imperative to implement a more uniform discovery approach by relying on a single criterion such as their shared dwarf galaxy environment. This is further motivated by two unambiguous cases of PRS associations with fast radio bursts (FRBs) which are luminous, millisecond-duration pulses of coherent radio emission with large dispersion measures pointing to an extragalactic provenance \citep{Lorimer07, Cordes19, Petroff22, Zhang23Review}. In particular, the first repeating FRB\,20121102A was pinpointed its location to a low-mass, dwarf host galaxy at $z = 0.1927$ \citep{Chatterjee17, Tendulkar17} and co-located with a compact ($\approx 1$~pc) PRS offset from the nucleus of the host galaxy \citep{Marcote17}. To date, several dozen FRBs have been localized to galaxies up to $z\sim1$ \citep{Heintz20,Gordon23, Law23} but only one other definitive FRB-PRS pair, FRB\,20190520B, has been discovered ($z = 0.241$; \citealt{Niu22}). We note that a third PRS was recently claimed to be associated with the active repeating FRB\,20201124A in a non-dwarf spiral host galaxy \citep{Xu22,Bruni23,Dong24}. However, the apparent offset of the PRS from the FRB location and a lack of conclusive evidence as to its compact nature makes this association more tentative.

%The combination of a PRS counterpart and its location in a dwarf galaxy has rendered FRB\,20190520B a close analog to FRB\,20121102A.


%The scarcity of multi-wavelength counterparts to FRBs despite dedicated follow-up efforts \citep{Scholtz16, Nunez21, Tavani21, Kilpatrick23, Law23} and the lack of any definitive evidence as to their origin further poses a challenge in illuminating the nature of their progenitors. 

%With only two robust FRB-PRS pairs, it is unclear whether PRSs represent a distinct sub-class of FRB progenitors.
%thus crucial to broaden the sample size, as they may represent a distinct sub-class in the FRB population and offer delineating power in the FRB progenitor channels. 
%Indeed, a recent search initiated by \cite{Vohl23} found a sample of luminous compact radio sources within dwarf galaxies at low redshifts ($z \lesssim 0.05$) with the LOw-Frequency ARray (LOFAR), thereby increasing the number of known dwarf PRSs.

%We find that the precise localization of FRB\,20211212A \citep{Gordon23}, does not align with its match Tier B source, J1027$+$0112, with a substantial spatial separation of $\approx$ 28\arcmin. As a result, we exclude FRB\,20211212A as a coincident FRB. For the remaining matches,  


hypernebula model

%We plot the evolutionary times in the left panel of Figure~\ref{fig:hypernebulae} for a range of mass-transfer rates $\dot{M}$ normalized to the Eddington accretion rate to trace out the critical timescales in the evolution of the hypernebula based on the assumed masses of the BH and donor star. The brown line denotes the maximum $t_{\rm active}$ of the system set by $M_\star$ and $\dot{M}$ (Equation~3 in \citealt{Sridhar+22}). %We now begin to constrain this parameter space with the observed size, luminosity, and radio SED of our Tier A source, J1136$+$2643. 

%Moreover, the SSA break frequency for J1136$+$2643 occurs at $\nu_{b}$ $\approx$ 3\,GHz when the shell is optically thick. Thus, using the turnover in the observed radio SED, we further eliminate the parameter space in which the optical depth of free-free absorption ($\tau_{\mathrm{ff}}$) for radio waves at 3\,GHz is $<1$. We mark this region in blue in Figure~\ref{fig:hypernebulae}. 
%The luminosity of the shock-heated electrons when the jet collides with the slower disk-wind shell is $L_{\rm e}\approx\varepsilon_{\rm e} L_{\rm j}$, where $\varepsilon_{\rm e}\sim0.5$ is the heating efficiency of the electrons \citep{Sironi&Spitkovsky_11} in an electron-ion shock with jet magnetization (the ratio of the magnetic enthalpy density to plasma enthalpy density) $\sigma_{\rm j}\sim 0.1$. We rule out the $\dot{M}$ range where the $L_{\rm e}\lesssim2\times10^{38}\,{\rm erg\,s^{-1}}$, corresponding to the observed radio luminosity at the turnover frequency in the red region. Finally, we rule out values of $\dot{M}$ and the ages of the system that yield inefficient synchrotron emission (i.e., a synchrotron cooling timescale $>$ the adiabatic cooling timescale; Equation~49 of \citealt{Sridhar+22}) in lilac in Figure~\ref{fig:hypernebulae}.

%\begin{equation}
%\begin{aligned} 
%L_{\rm w} & \approx\frac{1}{2}\dot{M}v_{\rm w}^2 \\
%& \approx 5\times10^{41}\,{\rm erg\,s^{-1}}\left(\frac{\dot{M}}{10^5\,\dot{M}_{\rm Edd}}\right)\left(\frac{M_\bullet}{10\,M_\star}\right)v_{\rm w,9}^2,
%\end{aligned}
%\end{equation}

%Although not consistent with the observed size of J1136$+$2643, this could potentially account for our Tier C sources, all of which are resolved out by VLBA observations. This is further supported by observations of large-scale ionized nebulae ($>$100\,pc; \citealt{Ramsey06, Grise11}) surrounding ultraluminous X-ray sources, exhibiting characteristics consistent with the energy output of massive outflows such as disk winds and collimated relativistic jets (e.g., \citealt{Pakull10, Soria21}) as posited by the model.


%in which the optical depth through the shell to free-free absorption for radio waves at 3\,GHz is $>1$ based on Equation~13 of \citealt{Sridhar+22} and the observed turnover in the radio SED (blue shaded region). Requiring that the synchrotron cooling timescale of heated electrons in the hypernebula be shorter than the adiabatic cooling timescale (Equation~49 of \citealt{Sridhar+22}) additionally rules out a region in the accretion rate-age phase space in which synchrotron emission is inefficient (lilac region). Here, we assume the jet magnetization to be $\sigma_{\rm j}=0.1$. 
%For high accretion rates of $\dot{M}/\dot{M}_{\rm Edd}$ = 10$^{5-6}$, the age of the hypernebula is constrained to $\lesssim$ 10\,yr. This age estimate is comparable with the derived values for PRSs\,20121102A, and 20190520B of $\sim$\,10 yr. This means that the putative hypernebula could be very young despite the fact that J1136$+$2643 is less luminous than the known FRB-PRSs as a high-$\dot{M}$ system implies a more luminous jet ($L_{j} \propto \dot{M}$). 


significantly higher than the average value in the ISM and the typical values in PWNe by at least 3 orders of magnitude \citep{Kothes06, Reynolds12}, however it is consistent with modeling of FRB-PRSs (e.g., \citealt{Margalit18}).


%Given the constraints mentioned above, we construct an `effective multi-zone' model for the observed radio synchrotron SED of J1136$+$2643. The model is constructed taking $\dot{M}/\dot{M}_{\rm Edd}=10^5$ and $t\approx 10$ yr. We first produce the radio synchrotron spectra from one-zone models by varying certain parameters between the range as mentioned above the right panel of Figure~\ref{fig:hypernebulae}. The final radio spectrum is generated by performing a weighted sum of the spectral curves from these one-zone models, following the methodology of \cite{Sridhar+22}. We justify the linear weighting of the models by the fact that the shock front may have different speeds and efficiencies at different regions, and the electrons are injected into the same nebula with different energies. The final weighted SED is shown as the dark grey curve in the right panel of Figure~\ref{fig:hypernebulae} superimposed on the observed radio SED of J1136$+$2643 (black dots). Also shown for comparison are the SEDs of the PRSs associated with FRBs\,20121102A, and 20190520B (denoted by maroon squares and red diamonds, respectively). The model reveals a satisfactory (admittedly tuned) proof-of-principle match to the SED of J1136$+$2643.

% {\it Right}: Radio synchrotron SED from the hypernebula model (grey curve) fit to the radio SED of J1136$+$2643 (black markers). The one-zone models are produced by varying the parameters between the ranges listed above the panel. The SEDs of the PRS associated with FRBs\,20121102A, and 20190520B are shown for comparison by the pentagon and diamond markers, respectively.

%\hspace{0.5cm}   
    %\includegraphics[width=0.5\textwidth]{images/PRS_dwarfgalaxis_hypernebula_tierA.pdf}

EVN: 
We observed 4 targets with the EVN and searched for bursts for a total of: 

3.38h: J0019+1507 (in text)
3.26h: J1027+0112 (in text)
2.84h : J1136+1252
3.32h : J0134-0741 (This is Fig7)

Total of: 12.8 hours


Our selection criteria for the EVN sample include 1) a minimum flux density of 2.5~mJy, 2) unresolved by the VLA, 3) a reliable redshift, and 4) when placed at the distance of FRB\,20121102A (z = 0.19), the compact radio sources have a comparable flux density to the PRS associated with FRB\,20121102A. 


INTRO:
%the formation of supermassive black holes (SMBHs) at the centers of galaxies has been a long standing question \citep{Rees84}. In models of black hole (BH) growth, IMBHs/AGN in low-redshift dwarf galaxies are sought after as relics of BH seeds, which provide the strongest constraints on the seed masses and hence the origin and growth of SMBHs (see \citealt{Reines16} for a review). 
%A radio study led by \cite{Reines20} has relied on the accretion signatures to identify the presence of IMBHs as off-nuclear wanderers. 

%(e.g., \citealt{GreenHo2004, Gallo08,  Reines13, Moran14, Sartori15})
%At close proximity ($\lesssim$ 10~Mpc), stellar and gas dynamics serve as effective tools to probe the presence of IMBHs in dwarf galaxies \citep{Lora09,Boyce17, Nguyen18, Nguyen19}. Moreover, numerous studies have relied on multiwavelength accretion signatures to gain demographic statistics on IMBHs, leading to the identification of hundreds of AGN candidates in dwarf galaxies \citep{Barth08, Reines13, Moran14, Sartori15,Baldassare20}, with some appearing as off-nuclear wanderers \citep{Mezcua20,Reines20}.


==> vlbiproperties.tex <==
\begin{table*}
\centering
\begin{tabular}{lccccc}
\hline
\hline
Source name & $z$  & Flux density & Luminosity\phantom{~~} & Angular size & Physical size \\
&  & (mJy) & (erg\,s$^{-1}$\,Hz$^{-1}$) & (mas) & (pc) \\
\hline
  J0019+1507  & 0.0376 & $1.3\pm0.2$ & $4.4 \times 10^{28}$& $< 4.6$ & $<3.5$ \\
  %J0134$-$0741 & 0.0156   &$10.0\pm1.5$ & $5.8 \times 10^{28}$ & $< 1.9$ & $<0.62$ \\
  J1027+0112  & 0.0212 & $2.8\pm0.4$& $3.0 \times 10^{28}$ & $< 2.0$ & $<0.89$ \\
  J1136+1252  & 0.0340 &$1.6\pm0.3$ & $4.4 \times 10^{28}$& $<1.3$ & $<0.91$ \\
 \hline
    \end{tabular}
    \caption{ Properties of the three sources detected with the EVN at 1.7\,GHz.  \label{tab:properties} }
\end{table*}
